Long Short-Term Memory for Early Warning Detection of Gravitational Waves

The pre-merger detection of gravitational waves from the early inspiral phase of compact binary coalescence events would allow the observation of the earlier stages of the merger in the electromagnetic band. This would significantly impact multi-messenger astronomy, giving astronomers potential access to rich new information. Here, we introduce a proof-of-concept deep-learning-based approach to produce pre-merger early-warning alerts for binary black hole systems. We show the possibility of using a Long Short-Term Memory network trained on the whitened detector strain in the time domain to detect and classify compact binary events. In this work, we consider a single advanced Laser Interferometer Gravitational-Wave Observatory detector at design sensitivity and make approximate sensitivity and early warning capability comparisons with approximations to traditional matched filtering approaches. We find that our model is competitive in both aspects, and when applied to a simulated test dataset was able to produce an early alert up to four seconds before the merger.

==> Backup.tex <==
\caption{This plot shows the predictive capability of LSTM model in detecting merger events prior to their actual occurrence, where the x-axis, labeled 'merger time', marks the precise time at which the mergers occur. The y-axis, labeled 'dt', indicates the amount of time in advance that the LSTM model can detect the signal before the merger takes place. Each point in the plot signifies an individual prediction instance, with the associated color representing the \acrshort{SNR} of the signals. \label{fig: 6.png}}

% ------------------
\subsection{Training the LSTM Model} \label{subsec: 4.2}

The LSTM model required 33 hours to fully train where each epoch takes 20 minutes on a single GPU. By analyzing the loss curves for the training and validation datasets, the model's performance was closely observed. The loss curves Fig. \ref{fig: 3} show that the findings were encouraging. Notably, the training loss curve showed a steady decline, indicating that the model was able to efficiently learn from the training set. Simultaneously, the validation loss curve descended in a manner akin to the training loss, with little deviation from it. This parallel fall shows that the model was not overfitting to the training set and is a sign of its ability to generalize, both curves' convergence towards lower loss values indicates that the model performed robustly, which is encouraging. where was able to identify the underlying patterns in the data. The training process, while thorough, has not yet reached convergence as indicated by the ongoing decrease in the loss curves. Further iterations may be required to achieve optimal performance. Additionally, the choices made regarding training parameters were deliberate; for instance, the batch size was selected to balance the computational load with the model's ability to generalize from the training data. The learning rate was chosen to ensure steady progress without overshooting the minima in the loss landscape, and the volume of training data was sufficient to represent the problem space without causing excessive training times or requiring prohibitive memory resources. These decisions were made with the intent to create a robust and efficient training regimen, tailored to the specific demands and limitations of our computational environment.

===================================

\begin{table}
\centering
\caption{Caption}
\begin{tabular}{c|c|c|c|c}
\hline \hline
Threshold Value & 6 & 8 & 10 &  LSTM with FAR 1 per day \\
\hline
  &  &  &  &  \\
Early warning detected by both  &  &  &  &  \\
Early Warning detected by LSTM only  &  &  &  &  \\
Early Warning Detected by CSNR only  &  &  &  &  \\
\hline \hline
\end{tabular}
\label{tab: 2}
\end{table}


========================================


\acro{GW}{Gravitational Wave}
\acro{BBH}{Binary Black Hole}
\acro{BNS}{Binary Neutron Star}
\acro{SNR}{Signal-to-Noise Ratio}
\acro{CSNR}{Cumulative Signal-to-Noise Ratio}
\acro{PSD}{Power Spectral Density}
\acro{CBC}{Compact Binary Coalescence}
\acro{LIGO}{Laser Interferometer Gravitational-Wave Observatory}
\acro{NSBH}{Neutron Star–Black Hole}
\acro{CNN}{Convolution Neural Network}
\acro{CLDNN}{Convolutional, Long Short-Term Memory, Fully-Connected Deep Neural Network Model}
\acro{RNN}{Recurrent Neural Network}
\acro{GRB}{Gamma-Ray Burst}
\acro{LSTM}{Long Short-Term Memory}
\acro{ROC}{Receiver Operating Characteristic}
\acro{EM}{Electromagnetic}
\acro{GWTC-3}{Third Gravitational-Wave Transient Catalogue}






The near-parallel performance of the matched filtering, especially in the low false alarm rate regime, underscores the \ac{LSTM}'s capability for effective signal classification and its promise as a computationally efficient alternative for real-time analysis.
